CyclicSim: Comprehensive Evaluation of Cyclic Shapers in Time-Sensitive Networking

Cyclic Queuing and Forwarding (CQF) is a key Time-Sensitive Networking (TSN) shaping mechanism that ensures bounded latency using a simple gate control list (GCL). Recently, variants of CQF, including Cycle Specific Queuing and Forwarding (CSQF) and Multi Cyclic Queuing and Forwarding (MCQF), have emerged. While popular TSN mechanisms such as the Time-Aware Shaper (TAS), Asynchronous Traffic Shaper (ATS), Credit-Based Shaper (CBS), and Strict Priority (SP) have been extensively studied, cyclic shapers have not been thoroughly evaluated. This paper presents a comprehensive analysis of CQF, CSQF, and MCQF, providing insights into their performance. We quantify delays through simulations and quantitative analysis on both synthetic and realistic networks. For the first time, we introduce an open-source OMNeT++ and INET4.4 based framework capable of modeling all three cyclic shaper variants. Our tool facilitates the validation of new algorithms and serves as a benchmark for cyclic shapers. Our evaluations reveal that MCQF supports diverse timing requirements, whereas CSQF, with its additional queue, often results in larger delays and jitter for some TT flows compared to CQF. Additionally, CSQF does not demonstrate significant advantages in TSN networks where propagation delays are less critical than in wide-area networks (WANs).

==> CCNC_2024_arxiv_camera_ready/reference.tex <==
@ARTICLE{8021Q,
  author={},
  journal={IEEE Std 802.1Q-2018 (Revision of IEEE Std 802.1Q-2014)}, 
  title={{IEEE} Standard for Local and Metropolitan Area Network--Bridges and Bridged Networks}, 
  year={2018},
  volume={},
  number={},
  pages={1-1993},
  doi={10.1109/IEEESTD.2018.8403927}}
  
@ARTICLE{8021Qbv,
  author={},
  journal={IEEE Std 802.1Qbv-2015 (Amendment to IEEE Std 802.1Q-2014 as amended by IEEE Std 802.1Qca-2015, IEEE Std 802.1Qcd-2015, and IEEE Std 802.1Q-2014/Cor 1-2015)}, 
  title={{IEEE} Standard for Local and metropolitan area networks -- Bridges and Bridged Networks - Amendment 25: Enhancements for Scheduled Traffic}, 
  year={2016},
  volume={},
  number={},
  pages={1-57},
  doi={10.1109/IEEESTD.2016.8613095}}
  
@ARTICLE{8021DG,
  author={},
  title={{P802.1DG} – {TSN} Profile for Automotive In-Vehicle Ethernet Communications}, 
  year={21 Dec 2021},
  volume={},
  number={},
  pages={}}
  
@ARTICLE{8021Qci,
  author={},
  journal={IEEE Std 802.1Qci-2017 (Amendment to IEEE Std 802.1Q-2014 as amended by IEEE Std 802.1Qca-2015, IEEE Std 802.1Qcd-2015, IEEE Std 802.1Q-2014/Cor 1-2015, IEEE Std 802.1Qbv-2015, IEEE Std 802.1Qbu-2016, and IEEE Std 802.1Qbz-2016)}, 
  title={IEEE Standard for Local and metropolitan area networks--Bridges and Bridged Networks--Amendment 28: Per-Stream Filtering and Policing}, 
  year={2017},
  volume={},
  number={},
  pages={1-65},
  doi={10.1109/IEEESTD.2017.8064221}}
  
@ARTICLE{8021Qcr,
  author={},
  journal={IEEE Std 802.1Qcr-2020 (Amendment to IEEE Std 802.1Q-2018 as amended by IEEE Std 802.1Qcp-2018, IEEE Std 802.1Qcc-2018, IEEE Std 802.1Qcy-2019, and IEEE Std 802.1Qcx-2020)}, 
  title={{IEEE} Standard for Local and Metropolitan Area Networks--Bridges and Bridged Networks - Amendment 34:Asynchronous Traffic Shaping}, 
  year={2020},
  volume={},
  number={},
  pages={1-151},
  doi={10.1109/IEEESTD.2020.9253013}}
  
@ARTICLE{60802,
  author={},
  journal={P60802 Standard for Local and Metropolitan Area Networks – Time-Sensitive Networking Profile for Industrial Automation}, 
  title={{IEC CD / IEEE 802.1 TSN} Time-Sensitive Networking Profile for Industrial Automation}, 
  author={IEEE},
  howpublished={\url{https://ieeexplore.ieee.org/document/9688733}},
  year={2023},
  note={Draft Version 2.0, accessed on May 1, 2023}}
  
@ARTICLE{8021AS,
  author={},
  journal={IEEE P802.1AS-Rev/D6.0 December 2017}, 
  title={IEEE Draft Standard for Local and Metropolitan Area Networks - Timing and Synchronization for Time-Sensitive Applications}, 
  year={2018},
  volume={},
  number={},
  pages={1-496},
  doi={}}
   
@ARTICLE{8021QAV,
  author={},
  journal={IEEE Std 802.1Qav-2009 (Amendment to IEEE Std 802.1Q-2005)}, 
  title={{IEEE} Standard for Local and Metropolitan Area Networks - Virtual Bridged Local Area Networks Amendment 12: Forwarding and Queuing Enhancements for Time-Sensitive Streams}, 
  year={2010},
  volume={},
  number={},
  pages={C1-72},
  doi={10.1109/IEEESTD.2009.5375704}}
  
@ARTICLE{8021BA,
  author={},
  journal={IEEE Std 802.1BA-2011}, 
  title={IEEE Standard for Local and metropolitan area networks--Audio Video Bridging {(AVB)} Systems}, 
  year={2011},
  volume={},
  number={},
  pages={1-45},
  doi={10.1109/IEEESTD.2011.6032690}}
  
  
@ARTICLE{8021Qbu,
  author={},
  journal={IEEE Std 802.1Qbu-2016 (Amendment to IEEE Std 802.1Q-2014)}, 
  title={{IEEE} Standard for Local and metropolitan area networks -- Bridges and Bridged Networks -- Amendment 26: Frame Preemption}, 
  year={2016},
  volume={},
  number={},
  pages={1-52},
  doi={10.1109/IEEESTD.2016.7553415}}

 @misc{iic_traffic,
  title={IIC TSN Testbed Traffic Whitepaper},
  author={Industrial Internet Consortium},
  howpublished={\url{https://www.iiconsortium.org/pdf/IIC_TSN_Testbed_Traffic_Whitepaper_20180418.pdf}},
  year={2018},
  note={[Online; accessed 1-May-2023]}
}

@misc{ademaj2018,
  title={Traffic Type Characterization for Time-Sensitive Networking},
  author={Ademaj, Astrit and Enzinger, Thomas},
  howpublished={\url{https://www.ieee802.org/1/files/public/docs2018/60802-ademaj-traffic-type-characterization-1118-v01.pdf}},
  year={2018},
  note={[Online; accessed 1-May-2023]}
}

@ARTICLE{mcqf_paul,
  author={Alexandris, Konstantinos and Pop, Paul and Wang, Tongtong},
  journal={IEEE Access}, 
  title={Configuration and Evaluation of {Multi-CQF} Shapers in {IEEE 802.1} {Time-Sensitive Networking (TSN)}}, 
  year={2022},
  volume={10},
  number={},
  pages={109068-109081},
  doi={10.1109/ACCESS.2022.3214007}}
  
  @INPROCEEDINGS{itp_infocom,
  author={Yan, Jinli and Quan, Wei and Jiang, Xuyan and Sun, Zhigang},
  booktitle={IEEE INFOCOM 2020 - IEEE Conference on Computer Communications}, 
  title={{Injection Time Planning}: Making {CQF} Practical in Time-Sensitive Networking}, 
  year={2020},
  volume={},
  number={},
  pages={616-625},
  doi={10.1109/INFOCOM41043.2020.9155434}}
  
  @article{survey_cqf_ahmed,
  author = {Ahmed Nasrallah and Venkatraman Balasubramanian and Akhilesh S. Thyagaturu and Martin Reisslein and Hesham Elbakoury},
  title = {Cyclic Queuing and Forwarding for Large Scale Deterministic Networks:{A} Survey},
  journal      = {CoRR},
  volume       = {abs/1905.08478},
  year         = {2019},
  url          = {http://arxiv.org/abs/1905.08478},
  eprinttype    = {arXiv},
  eprint       = {1905.08478},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1905-08478.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{tacq,
  author={Huang, Yudong and Wang, Shuo and Wu, Binwei and Huang, Tao and Liu, Yunjie},
  booktitle={ICC 2021 - IEEE International Conference on Communications}, 
  title={{TACQ}: Enabling Zero-jitter for Cyclic-Queuing and Forwarding in Time-Sensitive Networks}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/ICC42927.2021.9500914}}
  
  @ARTICLE{burst_aware_dong,
  author={Yang, Dong and Cheng, Zongrong and Zhang, Weiting and Zhang, Hongke and Shen, Xuemin},
  journal={IEEE/ACM Transactions on Networking}, 
  title={Burst-Aware Time-Triggered Flow Scheduling With Enhanced {Multi-CQF} in Time-Sensitive Networks}, 
  year={2023},
  volume={},
  number={},
  pages={1-16},
  doi={10.1109/TNET.2023.3264583}}
  
  @ARTICLE{drl_jrsp_mixed_flows_hao,
  author={Yu, Hao and Taleb, Tarik and Zhang, Jiawei},
  journal={IEEE Transactions on Industrial Informatics}, 
  title={Deep Reinforcement Learning based Deterministic Routing and Scheduling for Mixed-Criticality Flows}, 
  year={2022},
  volume={},
  number={},
  pages={1-11},
  doi={10.1109/TII.2022.3222314}}

@INPROCEEDINGS{jrs_cqf_yang,
  author={Liu, Yang and Cheng, Zongrong and Ren, Jie and Yang, Dong},
  booktitle={2022 7th International Conference on Computer and Communication Systems (ICCCS)}, 
  title={Joint Routing and Scheduling for {CQF}}, 
  year={2022},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/ICCCS55155.2022.9846349}}


@article{jrsp_ip_networks_jonatan,
title = {Joint routing and scheduling for large-scale deterministic {IP} networks},
journal = {Computer Communications},
volume = {165},
pages = {33-42},
year = {2021},
issn = {0140-3664},
doi = {https://doi.org/10.1016/j.comcom.2020.10.016},
url = {https://www.sciencedirect.com/science/article/pii/S0140366420319642},
author = {Jonatan Krolikowski and Sébastien Martin and Paolo Medagliani and Jérémie Leguay and Shuang Chen and Xiaodong Chang and Xuesong Geng}
}

@INPROCEEDINGS{mccqf_icc_yan,
  author={Liu, Yan and Zhou, Dajun and Zhan, Shuangping and Xin, Yao and Lin, Jiashuo and Feng, Xingbo and Shi, Enze and Qi, Ye and Chen, Gang and Zheng, Junqing and Wang, Yi and Zheng, Xiao},
  booktitle={ICC 2023 - IEEE International Conference on Communications}, 
  title={{MCCQF}: Low-Latency Transmission Based on {IEEE 802.1 Qch} For Hierarchical Networking}, 
  year={2023},
  volume={},
  number={},
  pages={6052-6058},
  doi={10.1109/ICC45041.2023.10279191}}


@INPROCEEDINGS{deepcqf_icc_cheng,
  author={Cheng, Zongrong and Yang, Dong and Zhang, Weiting and Ren, Jie and Wang, Hongchao and Zhang, Hongke},
  booktitle={ICC 2022 - IEEE International Conference on Communications}, 
  title={{DeepCQF}: Making {CQF} Scheduling More Intelligent and Practicable}, 
  year={2022},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/ICC45855.2022.9882280}}

@inproceedings{netcal_cqf_boyer,
  TITLE = {{A first Network Calculus model for Cyclic Queuing and Forwarding}},
  AUTHOR = {Guidolin--Pina, Damien and Boyer, Marc},
  URL = {https://hal.science/hal-04171262},
  BOOKTITLE = {{Junior Researcher Workshop on Real-Time Computing}},
  ADDRESS = {DORTMUND, Germany},
  YEAR = {2023},
  MONTH = Jun,
  PDF = {https://hal.science/hal-04171262/file/DTIS23092.1685016303.pdf},
  HAL_ID = {hal-04171262},
  HAL_VERSION = {v1},
}

@ARTICLE{jrs_cqf_transaction,
  author={Wang, Xiaolong and Yao, Haipeng and Mai, Tianle and Xiong, Zehui and Wang, Fu and Liu, Yunjie},
  journal={IEEE Transactions on Vehicular Technology}, 
  title={Joint Routing and Scheduling With Cyclic Queuing and Forwarding for Time-Sensitive Networks}, 
  year={2023},
  volume={72},
  number={3},
  pages={3793-3804},
  keywords={Logic gates;Routing;Job shop scheduling;Optimization;Switches;Schedules;Jitter;Time-sensitive networking (TSN);cyclic queuing and forwarding (CQF);joint routing and scheduling},
  doi={10.1109/TVT.2022.3216958}}

@ARTICLE{mss_transactions,
  author={Guo, Miao and Gu, Chaojie and He, Shibo and Shi, Zhiguo and Chen, Jiming},
  journal={IEEE Transactions on Industrial Informatics}, 
  title={{MSS}: Exploiting Mapping Score for {CQF} Start Time Planning in Time-Sensitive Networking}, 
  year={2023},
  volume={19},
  number={2},
  pages={2140-2150},
  doi={10.1109/TII.2022.3206815}}

@INPROCEEDINGS {tamcqf,
author = {H. Nie and S. Li and Y. Liu},
booktitle = {2023 IEEE Symposium on Computers and Communications (ISCC)},
title = {{TAMCQF}: Hybrid Traffic Scheduling Mechanism Integrating {TAS} and {Multi-CQF} in {TSN}},
year = {2023},
volume = {},
issn = {},
pages = {329-334},
doi = {10.1109/ISCC58397.2023.10218076},
url = {https://doi.ieeecomputersociety.org/10.1109/ISCC58397.2023.10218076},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {jul}
}

@ARTICLE{flexible_cqf_transaction,
  author={Huang, Yudong and Wang, Shuo and Zhang, Xinyuan and Huang, Tao and Liu, Yunjie},
  journal={IEEE Transactions on Network and Service Management}, 
  title={Flexible Cyclic Queuing and Forwarding for Time-Sensitive Software-Defined Networks}, 
  year={2023},
  volume={20},
  number={1},
  pages={533-546},
  doi={10.1109/TNSM.2022.3198171}}

@misc{ietfSegmentRouting,
    author = {Zhenqiang Li},
    title = {Segment Routing {(SR) }Based Bounded Latency},
    howpublished = {\url{https://datatracker.ietf.org/doc/html/draft-chen-detnet-sr-based-bounded-latency-01}},
    year = {},
    note = {[Accessed 04-02-2024]},
}

@misc{norman,
	author = {Finn, Norman},
	title = {Multiple Cyclic Queuing and Forwarding},
	howpublished = {\url{https://www.ieee802.org/1/files/public/docs2021/new-finn-multiple-CQF-0921-v02.pdf}},
	year = {2021},
	note = {[Accessed 04-02-2024]},
}

@ARTICLE{luxi_tnsm,
  author={Zhao, Luxi and Pop, Paul and Steinhorst, Sebastian},
  journal={IEEE Transactions on Network and Service Management}, 
  title={Quantitative Performance Comparison of Various Traffic Shapers in {Time-Sensitive Networking}}, 
  year={2022},
  volume={19},
  number={3},
  pages={2899-2928},
  doi={10.1109/TNSM.2022.3180160}}

@INPROCEEDINGS{rubi_rtcsa,
  author={Debnath, Rubi and Hortig, Philipp and Zhao, Luxi and Steinhorst, Sebastian},
  booktitle={2023 IEEE 29th International Conference on Embedded and Real-Time Computing Systems and Applications (RTCSA)}, 
  title={Advanced Modeling and Analysis of Individual and Combined {TSN} Shapers in {OMNeT++}}, 
  year={2023},
  volume={},
  number={},
  pages={176-185},
  doi={10.1109/RTCSA58653.2023.00029}}

@INPROCEEDINGS{rubi_noms,
  author={Debnath, Rubi and Hortig, Philipp and Zhao, Luxi and Steinhorst, Sebastian},
  booktitle={NOMS 2024-2024 IEEE Network Operations and Management Symposium}, 
  title={Quantifying the Impact of Frame Preemption on Combined TSN Shapers}, 
  year={2024},
  volume={},
  number={},
  pages={1-9},
  doi={10.1109/NOMS59830.2024.10575564}
}

@INPROCEEDINGS{rubi_vtc,
  author={Debnath, Rubi and Akinci, Mustafa Selman and Ajith, Devika and Steinhorst, Sebastian},
  booktitle={2023 IEEE 98th Vehicular Technology Conference (VTC2023-Fall)}, 
  title={{5GTQ}: {QoS-Aware} {5G-TSN} Simulation Framework}, 
  year={2023},
  volume={},
  number={},
  pages={1-7},
  doi={10.1109/VTC2023-Fall60731.2023.10333533}}

@ARTICLE{8021Qch,
  author={},
  journal={IEEE 802.1Qch-2017 (Amendment to IEEE Std 802.1Q-2014 as amended by IEEE Std 802.1Qca-2015, IEEE Std 802.1Qcd(TM)-2015, IEEE Std 802.1Q-2014/Cor 1-2015, IEEE Std 802.1Qbv-2015, IEEE Std 802.1Qbu-2016, IEEE Std 802.1Qbz-2016, and IEEE Std 802.1Qci-2017)}, 
  title={{IEEE} Standard for Local and metropolitan area networks--Bridges and Bridged Networks--Amendment 29: {Cyclic Queuing and Forwarding}}, 
  year={2017},
  volume={},
  number={},
  pages={1-30},
  doi={10.1109/IEEESTD.2017.7961303}}

@INPROCEEDINGS{qch_wang_performance,
  author={Wang, Bowen and Luo, Feng and Fang, Zihao},
  booktitle={2021 IEEE 4th International Conference on Computer and Communication Engineering Technology (CCET)}, 
  title={Performance Analysis of {IEEE} {802.1Qch} for Automotive Networks: Compared with {IEEE 802.1 Qbv}}, 
  year={2021},
  volume={},
  number={},
  pages={355-359},
  doi={10.1109/CCET52649.2021.9544333}}

@INPROCEEDINGS{online_qch_quan,
  author={Quan, Wei and Yan, Jinli and Jiang, Xuyan and Sun, Zhigang},
  booktitle={2020 IEEE 22nd International Conference on High Performance Computing and Communications; IEEE 18th International Conference on Smart City; IEEE 6th International Conference on Data Science and Systems (HPCC/SmartCity/DSS)}, 
  title={On-line Traffic Scheduling optimization in {IEEE} {802.1Qch} based {Time-Sensitive Networks}}, 
  year={2020},
  volume={},
  number={},
  pages={369-376},
  doi={10.1109/HPCC-SmartCity-DSS50907.2020.00045}}

@INPROCEEDINGS{assessment_qch_leonardi,
  author={Leonardi, Luca and Bello, Lucia Lo and Patti, Gaetano},
  booktitle={2020 AEIT International Conference of Electrical and Electronic Technologies for Automotive (AEIT AUTOMOTIVE)}, 
  title={Performance assessment of the {IEEE 802.1Qch} in an automotive scenario}, 
  year={2020},
  volume={},
  number={},
  pages={1-6},
  doi={10.23919/AEITAUTOMOTIVE50086.2020.9307422}}

@ARTICLE{config_offset_damien,
  author={Guidolin–Pina, Damien and Boyer, Marc and Boudec, Jean-Yves Le},
  journal={IEEE/ACM Transactions on Networking}, 
  title={Configuration of Guard Band and Offsets in Cyclic Queuing and Forwarding}, 
  year={2023},
  volume={},
  number={},
  pages={1-0}}

@INPROCEEDINGS{deepscheduler,
  author={He, Xiaowu and Zhuge, Xiangwen and Dang, Fan and Xu, Wang and Yang, Zheng},
  booktitle={IEEE INFOCOM 2023 - IEEE Conference on Computer Communications}, 
  title={{DeepScheduler}: Enabling Flow-Aware Scheduling in {Time-Sensitive Networking}}, 
  year={2023},
  volume={},
  number={},
  pages={1-10},
  doi={10.1109/INFOCOM53939.2023.10228875}}

@ARTICLE{cqf_fp,
  author={Luo, Feng and Wang, Zitong and Guo, Yi and Wu, Mingzhi and Feng, Wanqiang and Sun, Zhipeng},
  journal={IEEE Embedded Systems Letters}, 
  title={Research on Cyclic Queuing and Forwarding with Preemption in Time-Sensitive Networking}, 
  year={2023},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/LES.2023.3292833}}


@ARTICLE{simulation_cqf_fp,
  author={Luo, Feng and Wang, Zitong and Ren, Yi and Wu, Mingzhi and Zhang, Xiaoxian},
  journal={SAE Technical Paper 2024-01-1986, 2024}, 
  title={Simulative Assessments of Cyclic Queuing and Forwarding with Preemption in In-Vehicle Time-Sensitive Networking}, 
  year={2023},
  volume={},
  number={},
  pages={1-1},
  doi={https://doi.org/10.4271/2024-01-1986}}

@article{tamcqf_2024,
author = {Nie, Hongrui and Su, Yue and Zhao, Weibo and Mu, Junsheng},
title = {Hybrid traffic scheduling in time-sensitive networking for the support of automotive applications},
journal = {IET Communications},
volume = {18},
number = {2},
pages = {111-128},
year = {2024}
}

@misc{arxiv_sch_survey,
      title={Schedulability Analysis in Time-Sensitive Networking: A Systematic Literature Review}, 
      author={Zitong Wang and Feng Luo and Yunpeng Li and Haotian Gan and Lei Zhu},
      year={2024},
      eprint={2407.15031},
      archivePrefix={arXiv},
      primaryClass={cs.NI},
      url={https://arxiv.org/abs/2407.15031}, 
}

@INPROCEEDINGS{fits_quan,
  author={Quan, Wei and Yan, Jinli and Jiang, Xuyan and Sun, Zhigang},
  booktitle={2020 IEEE 22nd International Conference on High Performance Computing and Communications; IEEE 18th International Conference on Smart City; IEEE 6th International Conference on Data Science and Systems (HPCC/SmartCity/DSS)}, 
  title={On-line Traffic Scheduling optimization in IEEE 802.1Qch based Time-Sensitive Networks}, 
  year={2020},
  volume={},
  number={},
  pages={369-376},
  doi={10.1109/HPCC-SmartCity-DSS50907.2020.00045}}

@INPROCEEDINGS{leonardi_qch_sim,
  author={Leonardi, Luca and Bello, Lucia Lo and Patti, Gaetano},
  booktitle={2020 AEIT International Conference of Electrical and Electronic Technologies for Automotive (AEIT AUTOMOTIVE)}, 
  title={Performance assessment of the IEEE 802.1Qch in an automotive scenario}, 
  year={2020},
  volume={},
  number={},
  pages={1-6},
  doi={10.23919/AEITAUTOMOTIVE50086.2020.9307422}}

@ARTICLE{ahmed_access,
  author={Nasrallah, Ahmed and Thyagaturu, Akhilesh S. and Alharbi, Ziyad and Wang, Cuixiang and Shao, Xing and Reisslein, Martin and Elbakoury, Hesham},
  journal={IEEE Access}, 
  title={Performance Comparison of {IEEE} 802.1 TSN Time Aware Shaper ({TAS}) and Asynchronous Traffic Shaper ({ATS})}, 
  year={2019},
  volume={7},
  number={},
  pages={44165-44181},
  doi={10.1109/ACCESS.2019.2908613}}

@INPROCEEDINGS{anna_fp,
  author={Arestova, Anna and Jens Hielscher, Kai-Steffen and German, Reinhard},
  booktitle={2021 IFIP Networking Conference (IFIP Networking)}, 
  title={Simulative Evaluation of the TSN Mechanisms Time-Aware Shaper and Frame Preemption and Their Suitability for Industrial Use Cases}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.23919/IFIPNetworking52078.2021.9472830}}

@article{cqf_survey_ahmed,
  author = {Ahmed Nasrallah and
                  Venkatraman Balasubramanian and
                  Akhilesh S. Thyagaturu and
                  Martin Reisslein and
                  Hesham Elbakoury},
  title = {Cyclic Queuing and Forwarding for Large Scale Deterministic Networks:
                  {A} Survey},
  journal      = {CoRR},
  volume       = {abs/1905.08478},
  year         = {2019}
}

@INPROCEEDINGS{iecon_cqf,
  author={Luo, Feng and Guo, Yi and Wang, Zitong and Yang, Zhenyu and Ren, Yi and Wang, Jiajia and Zhang, Ping},
  booktitle={IECON 2023- 49th Annual Conference of the IEEE Industrial Electronics Society}, 
  title={Analysis of the Performance Advantage of Cyclic Queuing and Forwarding Mechanism in Vehicle Time-Sensitive Network}, 
  year={2023},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/IECON51785.2023.10311699}
}

@inproceedings {nesting_2019,
    author = {Jonathan Falk and David Hellmanns and Ben Carabelli and Naresh Nayak and Frank D{\"u}rr and Stephan Kehrer and Kurt Rothermel},
    title = {{NeSTiNg}: Simulating {IEEE} Time-sensitive Networking ({TSN}) in {OMNeT}++},
    booktitle = {Proceedings of the 2019 International Conference on Networked Systems (NetSys)},
    address = {Garching b. M{\"u}nchen, Germany},
    month = mar,
    year = {2019},
} 

@Inbook{Meyer2019,
author="Meyer, Philipp
and Korf, Franz
and Steinbach, Till
and Schmidt, Thomas C.",
editor="Virdis, Antonio
and Kirsche, Michael",
title="Simulation of Mixed Critical In-Vehicular Networks",
bookTitle="Recent Advances in Network Simulation: The OMNeT++ Environment and its Ecosystem",
year="2019",
publisher="Springer International Publishing",
address="Cham",
pages="317--345",
isbn="978-3-030-12842-5",
doi="10.1007/978-3-030-12842-5_10",
url="https://doi.org/10.1007/978-3-030-12842-5_10"
}


@Article{sensors_cqf,
AUTHOR = {Luo, Feng and Wang, Bowen and Yang, Zhenyu and Zhang, Ping and Ma, Yifei and Fang, Zihao and Wu, Mingzhi and Sun, Zhipeng},
TITLE = {Design Methodology of Automotive Time-Sensitive Network System Based on {OMNeT++} Simulation System},
JOURNAL = {Sensors},
VOLUME = {22},
YEAR = {2022},
NUMBER = {12},
ARTICLE-NUMBER = {4580}
}

@article{reusch2023configuration,
  title={Configuration optimization for heterogeneous time-sensitive networks},
  author={Reusch, Niklas and Barzegaran, Mohammadreza and Zhao, Luxi and Craciunas, Silviu S and Pop, Paul},
  journal={Real-Time Systems},
  volume={59},
  number={4},
  pages={705--747},
  year={2023},
  publisher={Springer}
}

